CapEst: A Measurement-based Approach to Estimating Link Capacity in Wireless Networks

Estimating link capacity in a wireless network is a complex task because the available capacity at a link is a function of not only the current arrival rate at that link, but also of the arrival rate at links which interfere with that link as well as of the nature of interference between these links. Models which accurately characterize this dependence are either too computationally complex to be useful or lack accuracy. Further, they have a high implementation overhead and make restrictive assumptions, which makes them inapplicable to real networks. In this paper, we propose CapEst, a general, simple yet accurate, measurement-based approach to estimating link capacity in a wireless network. To be computationally light, CapEst allows inaccuracy in estimation; however, using measurements, it can correct this inaccuracy in an iterative fashion and converge to the correct estimate. Our evaluation shows that CapEst always converged to within 5% of the correct value in less than 18 iterations. CapEst is model-independent, hence, is applicable to any MAC/PHY layer and works with auto-rate adaptation. Moreover, it has a low implementation overhead, can be used with any application which requires an estimate of residual capacity on a wireless link and can be implemented completely at the network layer without any support from the underlying chipset.

==> define.tex <==
\section{Wireless Link Capacity}
\label{sec:define}

% would have defined wireless link capacity in the introduction.....
In this section, we use examples to demonstrate why building a model to accurately estimate capacity is so hard.
Consider link $4 \rightarrow 5$ in Figure~\ref{fig:fim}. We first assume that no other link in this topology is transmitting. 
If $C$ Mbps denotes the data rate on link $4 \rightarrow 5$ and $x$ denotes the proportion of time wasted due to overhead (which includes
the time wasted in transmitting control messages like IEEE 802.11 ACK as well as the time wasted in random back-offs), the link capacity of 
$4 \rightarrow 5$ is equal to $\left( 1 - x \right) C$ Mbps (Figure~\ref{fig:define}). 

Now, lets assume that there is a transmission going on at link $5 \rightarrow 6$ for $y$ proportion of time. A transmission
on this link will force node $4$ to freeze its state due to virtual carrier sensing, hence, transmissions on link $5 \rightarrow 6$
will eat up the capacity in link $4 \rightarrow 5$. Ideally, the capacity of link $4 \rightarrow 5$ should reduce to $\left( 1 - x - y\right) C$ Mbps.
However, random access scheduling can result in data transmissions on links $4 \rightarrow 5$ and $5 \rightarrow 6$ colliding which will reduce
the net capacity on link $4 \rightarrow 5$. And this reduction is a non-linear function of $y$ (Figure~\ref{fig:define}). 

Now, lets assume that there is a transmission going on at link $2 \rightarrow 3$ for $y$ proportion of time (and link $5 \rightarrow 6$ is silent).
Any transmission on this link will cause the data transmission on link $4 \rightarrow 5$ to collide, and hence, will reduce the net capacity
of this link. And this reduction in capacity is not only a non-linear, non-convex function of $y$, but is also different from the capacity reduction 
resulting due to link $5 \rightarrow 6$ transmitting for $y$ proportion of time (Figure~\ref{fig:define}).
Thus, the same number of transmissions on different neighboring links affect the capacity on a wireless link differently and non-linearly.
Hence, in a manner similar to the methodology proposed in~\cite{}, 
using a simple linear equation like $\sum_{k \rightarrow l \in N_{i \rightarrow j}} \lambda_{k \rightarrow l} \leq \left( 1 - x \right) C$, $\forall$ links $i \rightarrow j$,
where $\lambda_{kl}$ denotes the rate on link $k \rightarrow l$, $C$ is the data rate at all links, $x$ is the proportion of time wasted in overhead
and $N_{i \rightarrow j}$ denotes the set of links which interfere with $i \rightarrow j$ will either overestimate or underestimate capacity.

Now, finally lets assume that there is a transmission going an at links $2 \rightarrow 3$ and $8 \rightarrow 9$ for $y/2$ proportion of time each. 
A first glance, it may seem that a total of $y$ proportion of time is being used to transmit data on the neighboring links of $4 \rightarrow 5$. 
However, links $2 \rightarrow 3$ and $8 \rightarrow 9$ do not interfere with each other and can be scheduled simultaneously. 
Then, does the capacity reduce to a scenario where $y/2$ proportion of time is being used to transmit data on the neighboring links of $4 \rightarrow 5$. 
And the answer is no because IEEE 802.11 schedules these two non-interfering links independently, hence, there will be times when none of these three
links is transmitting. Hence, how much does the capacity reduce cannot be determined easily and the simple linear 
described above can be extremely inaccurate in such a scenario. And how much does this capacity reduce cannot be even accurately represented
through a system of convex equations. 

Finally, from the above discussion it seems that the capacity at a link depends only on the input rate at neighboring edges. 
This deduction is not true either. Consider Figure~\ref{fig:chain_cross}. Links $2 \rightarrow 3$ and $6 \rightarrow 7$ do not interfere with each other. 
However, increasing the number of transmissions of flow $6 \rightarrow 7$ will reduce the capacity on link $2 \rightarrow 3$. 
More transmissions on link $6 \rightarrow 7$ will cause more collisions on link $4 \rightarrow 5$ which will increase the actual number 
of transmissions occurring on this link (due to retransmissions) which will cause more collisions on link $2 \rightarrow 3$ which will
reduce its capacity. Thus, every pair of links in a network, interfering or non-interfering, will impact each other's capacity in a non-linear, non-convex fashion.
This will make a model, which can be used to accurately determine capacity at a link, so complex that it may no longer remain useful.
Thus, instead of spending our effort on building a complex but accurate model or simple or inaccurate model to represent the system, 
we will focus on building a methodology which will give an inaccurate capacity estimate the first time around, however, it will keep updating
the capacity estimate over time and will iteratively converge to the correct capacity value. 

An important point to note here is that the capacity at a link is eaten only by transmissions on neighboring edges. 
In other words, a non-interfering link $k \rightarrow l$ impacts the the number of transmissions on an interfering link
for $i \rightarrow j$, and hence, impacts the capacity at link $i \rightarrow j$. Thus, any extra capacity available at
$i \rightarrow j$ will have to be distributed only amongst transmissions on those links which interfere with $i \rightarrow j$.
This important observation will significantly simplify the design of CapEst. 



==> outline.tex <==
\section{Outline}

1. Introduction.
 - Wireless Networking and all the problems and why require capacity estimation.
 - Why is it hard? 
   - Capacity of a link eaten up by neighbors too.
   - Use the flow in the middle topology example to show the capacity region.
   - Capacity eating is not linear. A complex function of rates on all the edges and the topology.
 - Can we do capacity estimation with the following constraints.
    - No topology information (how do edges interfere, carrier sensing probs and capture probs etc) expensive to collect.   
    - Should be MAC and PHY independent. MAC and PHY are ever changing. If we create a mode like others, will be applicable to only one. 
    - Simple measurements. No assumption on the firmware driver.Like busy probability.
    - Robust to dynamics. Any change in the topology or interference characteristics should be easily and automatically taken care of.
 - A simple mechanism to estimate capacity based on measuring the expected service time per edge. 
   - Iteratively converge to the correct capacity estimate. 
 - Use a simple application of online optimization to demonstrate that the technique is able to accurately estimate capacity. 
 - Different applications to showcase the proposed technique.
   - Distributed rate allocation. 
   - Admission Control.
 - Organization.


2. Define what we mean by wireless link capacity using the flow in the middle example.

3. Mechanism.
 A Describe the mechanism to estimate capacity.
 B Briefly summarize the mechanism to divide capacity to get max-min fairness.

4. Convergence
 - State an analytical theorem to state the assumptions and the result. 

5. Validation
 - Study convergence for a number of topologies, different MACs, finite retransmit limits, auto-rate adaptation.
 - Also study convergence with experiments.

6. Applications
 A Online optimization
  - Define. 
  - Show weighted max-min fairness.
  - Compare with Sigcomm'08 and CoNext'09.
 B Distributed Rate Allocation 
  - Describe WCPCap with the new estimation technique.
  - Compare throughputs for FIM and chain-cross.
 C Admission Control 
  - Describe the problem and define a metric.
  - Compare for Houson topology and chain-cross.

7. Related Work
 A Other capacity estimation techniques
  - Model-based.
  - Other expected service time based, but are end-to-end. Not neighborhood based. 
 B Other rate allocation mechanisms. Alternatives of TCP, or capacity estimation technique is a heuristic which may not yield good throughputs. 
 C Jointly optimizing transport and scheduling. (Backpressure-based algorithms).

8. Conclusions

